Strong Typed B\"ohm Theorem and Functional Completeness on the Linear Lambda Calculus

In this paper, we prove a version of the typed B\"ohm theorem on the linear lambda calculus, which says, for any given types A and B, when two different closed terms s1 and s2 of A and any closed terms u1 and u2 of B are given, there is a term t such that t s1 is convertible to u1 and t s2 is convertible to u2. Several years ago, a weaker version of this theorem was proved, but the stronger version was open. As a corollary of this theorem, we prove that if A has two different closed terms s1 and s2, then A is functionally complete with regard to s1 and s2. So far, it was only known that a few types are functionally complete.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Atkey \& Krishnaswami (Eds.): MSFP 2016\\
EPTCS 207, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.207.1}{10.4204/EPTCS.207.1}}

